LambdaKG: A Library for Pre-trained Language Model-Based Knowledge Graph Embeddings

Knowledge Graphs (KGs) often have two characteristics: heterogeneous graph structure and text-rich entity/relation information. Text-based KG embeddings can represent entities by encoding descriptions with pre-trained language models, but no open-sourced library is specifically designed for KGs with PLMs at present. In this paper, we present LambdaKG, a library for KGE that equips with many pre-trained language models (e.g., BERT, BART, T5, GPT-3), and supports various tasks (e.g., knowledge graph completion, question answering, recommendation, and knowledge probing). LambdaKG is publicly open-sourced at https://github.com/zjunlp/PromptKG/tree/main/lambdaKG, with a demo video at http://deepke.zjukg.cn/lambdakg.mp4 and long-term maintenance.

==> charts/lama_probe.tex <==
\let\mc\multicolumn

\begin{table}[thbp]
\small

\label{tb:lama-probe}
\centering
\setlength{\tabcolsep}{5mm}
{% <------ Don't forget this %
\begin{tabular}{lccc}

% \setlength{\tapcolsep}{4cm}
\toprule
Model & \mc{2}{c}{LAMA} \\
 \cmidrule(lr){2-3}
& hits1 & MRR \\
\midrule 
BERT-base & 62.4 & 57.0 \\
$k$NN-KGE & 52.5 & 57.9  \\
% \midrule 

\bottomrule
\end{tabular}
}%
\caption{LAMA probe result.}
% \label{tb:time}
\end{table}

==> charts/link_prediction.tex <==
\let\mc\multicolumn

\begin{table}[thbp]
\small

\label{tb:link-prediction}
\centering
% \setlength{\tabcolsep}{5mm}
{% <------ Don't forget this %
\begin{tabular}{lcccc}

% \setlength{\tapcolsep}{4cm}
\toprule
Model & \mc{2}{c}{WN18RR} & \mc{2}{c}{FB15k-237} \\
 \cmidrule(lr){2-3}  \cmidrule(lr){4-5}  
& hits1 & MRR & hits1 & MRR \\
\midrule 
KGBERT & 4.1 & 21.6 & - & - \\
$k$NN-KGE & 52.5 & 57.9 & 28.0 & 37.0 \\
SimKGC & 58.5 & 67.1 & 24.6 & 33.3\\
StAR & 24.3 & 40.1 & 20.5 & 29.6\\
KGT5 & 48.7 & 50.8 & 21.0 & 27.6\\
GenKGC & 28.7 & - & 19.2 & -\\
% \midrule 

\bottomrule
\end{tabular}
}%
% TODO 搞定 3090 真实时间
\caption{Link prediction result.}
% \label{tb:time}
\end{table}

==> images/diff_PLMs.tex <==

\begin{figure}[!t] %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
\centering %图片居中

\includegraphics[width=0.4\textwidth]{./resources/result.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
\caption{
Performance of \ours \ with different PLMs. }
\label{fig:diff_PLMs}
\end{figure}


